Quantifying Feature Space Universality Across Large Language Models via Sparse Autoencoders

The Universality Hypothesis in large language models (LLMs) claims that different models converge towards similar concept representations in their latent spaces. Providing evidence for this hypothesis would enable researchers to exploit universal properties, facilitating the generalization of mechanistic interpretability techniques across models. Previous works studied if LLMs learned the same features, which are internal representations that activate on specific concepts. Since comparing features across LLMs is challenging due to polysemanticity, in which LLM neurons often correspond to multiple unrelated features rather than to distinct concepts, sparse autoencoders (SAEs) have been employed to disentangle LLM neurons into SAE features corresponding to distinct concepts. In this paper, we introduce a new variation of the universality hypothesis called Analogous Feature Universality: we hypothesize that even if SAEs across different models learn different feature representations, the spaces spanned by SAE features are similar, such that one SAE space is similar to another SAE space under rotation-invariant transformations. Evidence for this hypothesis would imply that interpretability techniques related to latent spaces, such as steering vectors, may be transferred across models via certain transformations. To investigate this hypothesis, we first pair SAE features across different models via activation correlation, and then measure spatial relation similarities between paired features via representational similarity measures, which transform spaces into representations that reveal hidden relational similarities. Our experiments demonstrate high similarities for SAE feature spaces across various LLMs, providing evidence for feature space universality.

==> emnlp_vers/texs/1_intro.tex <==
\section{Introduction}

Large language models (LLMs) have demonstrated remarkable capabilities across a wide range of natural language tasks \citep{bubeck2023sparksartificialgeneralintelligence, naveed2024comprehensiveoverviewlargelanguage, Liu_2023}. However, understanding how these models internally represent information remains a significant challenge \citep{bereska2024mechanisticinterpretabilityaisafety}. 
% , which would shed light on if each model develops mostly dissimilar ways of encoding linguistic knowledge. 
The \emph{Universality Hypothesis} claims that different models converge towards similar concept representations in their latent spaces \citep{huh2024platonic}. Providing evidence for this hypothesis would enable researchers to exploit universal properties related to features, providing new ways for generalizating mechanistic interpretability techniques across models \citep{apollo2024mechinterp}, and accelerating research towards safer, more controllable AI systems \citep{hendrycks2023overviewcatastrophicairisks}.

% Several works have studied if LLMs learn the same features
If LLMs learn similar internal concept representations, called \emph{features}, it is vital is to understand which measures they are similar under, and to quantify the extent of these similarities \citep{ChughtaiToy, gurnee2024universalneuronsgpt2language}. Since comparing features across LLMs is challenging due to polysemanticity, in which individual neurons often correspond to multiple unrelated features, rather than to distinct concepts, sparse autoencoders (SAEs) have been employed to disentangle polysemantic LLM neurons into SAE features corresponding to distinct concepts that are easier to analyze  \citep{cunningham2023sparseautoencodershighlyinterpretable}. 
Previous works found that while SAEs learn similar features, they also learn a notable percentage of different features that are idiosyncratic to specific SAEs \citep{leask2025sparse, paulo2025sparseautoencoderstraineddata}. Even so, SAEs across models learn correlated features which activate on the same concepts \citep{bricken2023monosemanticity}. Moreover, semantically similar SAE feature arrangements are found across SAEs trained on different models, such as "months" features arranged circularly in GPT-2, Mistral-7B, and Llama-3 8B \citep{engels2024languagemodelfeatureslinear, leask2024calendar}. Research has also found other types of feature arrangements \citep{park2024geometry, Li_2025, oneill2024disentanglingdenseembeddingssparse}. 
These findings suggest  a new way of investigating universality based on feature relations.
% These findings suggest investigating a new type of universality based on feature relations.

In this paper, we introduce a new variation of the universality hypothesis called  \textbf{Analogous Feature Universality}: we hypothesize that even if SAEs across different models learn different feature representations, the spaces spanned by SAE features are similar, such that one SAE space is similar to another SAE space under certain rotation-invariant transformations.
Evidence supporting this hypothesis would imply that latent spaces may have similar geometric arrangements of semantic subspaces \citep{templeton2024scaling}, suggesting that features, and techniques related to feature spaces (e.g. steering vectors), may be transferred across models via particular transformations. Features have been transferred across models \citep{merullo2023linearlymappingimagetext}, but there is a lack of research explaining why this can be done.

% wang2018understanding, 
To investigate this hypothesis, we develop a novel approach that involves two main steps: (1) first, we pair SAE features across different models via activation correlation, and (2) afterwards, we measure the similarity of spatial relations between paired features using representational space similarity measures, which transform spaces into representations that reveal hidden relational similarities \citep{Raghu2017SVCCASV, Kriegeskorte2008}. 
This approach addresses a different research question compared to previous representational similarity papers \citep{kornblith2019similarityneuralnetworkrepresentations, klabunde2024resicomprehensivebenchmarkrepresentational, klabunde2023similarityneuralnetworkmodels, SucholutskyAligned}, which \textbf{did not measure the relationships among features}, but among \emph{input data samples} that were already known to correspond to the “same point” in input data space. In contrast, to investigate our hypothesis, our approach differs from previous approaches as it introduces step 1, which allows us to assess if we can use features, not input samples, to determine if representations are the same across models. Thus, we are applying representational similarity \emph{based on features in weight space}, instead of based on input data samples in activation space. 
% These scores would only show notable similarities if the features are paired correctly.

% If correlated feature pairs beget high similarity scores, then these correlated features would 
To better describe why this approach works for testing our hypothesis, we can consider the following analogy: given three points [1, 2, 3] on a right triangle, we can think of each point like a feature. One model may label these points as [A, B, C], with each position being a column of a matrix, and another model may label them as [X, Y, Z]. However, these points are not ordered the same in each matrix, so we may find them in the order of [B, C, A] and [Z, X, Y]. But if we rearrange them into pairs “close enough to” [1, 2, 3] by estimating which points they correspond to on a right triangle, then we can align the two representations, and measure if the relationship among them---a right triangle---is also similar. This necessitates step 1 in our approach: consistent high scores across models can only be found if features are paired correctly. 
% \footnote{Appendix ! and Figure ! elaborate on this topic. \hl{TBD}}
% a high score for correlated features indicates that even if the features are different, 
% make figure
% , like (A, X),

% To verify the effectiveness of our approach, we present a comprehensive set of experiments and results across models with varying architectures, sizes, and training regimes. Our experimental approach involves solving two issues for representational space similarity measurement: the permutation issue, which involves aligning individual neurons, and the rotational issue, which involves comparing two spaces which have different basis that are rotationally-invariant. 
% Additionally, we present an approach to filter out feature matches with low semantically-meaningful similarity.

Our experiments demonstrate high similarities in SAE feature spaces between middle layers across multiple LLMs, providing evidence for feature space universality. 
Furthermore, we show that semantically meaningful subspaces exhibit notable similarity across models. 
% (e.g., features related to specific concepts, such as Emotions) 
% We also analyze how feature similarity varies across different layers of LLMs, revealing patterns in how representations evolve through the model depth.

% Additionally, our results reveal the differences in features which are not captured by SAEs. While we discover evidence that LLMs learn weakly universal features, and that SAEs can capture both these features and these relations, we also find that different SAEs do not consistently learn the same exact features captured by LLMs, a finding that is supported by previous work \citep{leask2025sparse, paulo2025sparseautoencoderstraineddata}. Thus, our research guides future work to improve upon methods that can better capture universal representations of features \citep{thasarathan2025universalsparseautoencodersinterpretable}, and contributes to ongoing research that aims to improve SAEs \citep{engels2024decomposingdarkmattersparse}. 
\textbf{Our key contributions include:}
\begin{enumerate}

\item Empirical evidence for similar SAE feature space representations across diverse LLMs. 
% Previously, SAE feature similarity was only studied in 1L toy models.

\item A novel approach to study similar feature spaces by comparing weight representations, instead of activation representations, via paired features.

\item An in-depth analysis of how feature similarity varies by semantic subspaces (e.g. Emotions).

\end{enumerate}

% Because LLMs, even with the same architecture, can learn many different features, we do not expect entire feature spaces to be highly similar; instead, we hypothesize there may be highly similar \emph{subspaces}. In other words, there are many similar features universally found across SAEs, but not every feature learned by different SAEs is the same.

% \textbf{Motivation and Impact}: If SAEs do not learn similar feature spaces, then SAE interpretability discoveries, such as feature circuits, would be confined to one model. But if they learn similar feature spaces, then these findings can generalize across models.
% The discovery of "canonical features" or "canonical feature relations" that recur throughout multiple models may accelerate sparse dictionary learning, as identifiable patterns or features can be isolated and emphasized during training, allowing the model to hone in faster on key concepts \citep{apollo2024mechinterp}. Additionally, if we compare the activations of dangerous models vs safe models, both in the original space and SAE feature space, we may be able to diagnose issues in these models and steer them to safer states. We can identify universally dangerous feature patterns that were not able to be found in the original LLM space due to superposition.

% \textbf{Importance of Representational Similarity. } Finding similar semantically meanigful spaces is a stronger criteria as it shows that models are not just capturing similar discrete concepts, but continuous spaces of concepts, which carry information on how concepts are arranged relative to one another. If only individual features were similar, but not feature relations, then techniques such as steering vectors, which rely on difference-of-means between concepts, may not generalize as well.
% By finding universal patterns of feature subspaces, we can generalize feature relations across models, such as not just knowing that two models each have the concepts of 'king' and 'queen', but that they both similarly represent the entire subspace of royalty that includes king-queen-princess-crown and more. 

\begin{figure*}[!ht]
  \centering
  \includegraphics[scale=0.4]{diagrams/fig1.pdf}
  \caption{We train SAEs on LLMs, and then compare their SAE feature space similarity using measures such as Singular Value Canonical Correlation Analysis (SVCCA). }
  \label{fig:summary_temp}
\end{figure*}

% \textcolor{red}{show that the SAE a and B are not aligned before SVCCA?}
% % 2 LLMs with mapping score, and 2 SAEs on one of their layers with another mapping score. 

% (added new line to discuss this in first paragraph of Methodology: "For the rotational issue, models typically develop their own basis for latent space representations, so features may be similar relation-wise across spaces, but not rotation-wise due to differing basis.")

==> emnlp_vers/texs/2_background.tex <==
\section{Background and Definitions} %  and Related Work

\textbf{Feature Universality.} We define a feature as an internal representation that activates on a concept \citep{park2024linear}. To quantify the extent of feature space universality, we utilize the following definitions that build on terms defined in previous works:
We define \textbf{correlated features} as features which are correlated in terms of activation similarity, and thus activate highly on the same tokens \citep{bricken2023monosemanticity}. We measure the \textbf{representational universality} of feature spaces by applying representational similarity measures on a set of correlated feature pairs \citep{gurnee2024universalneuronsgpt2language}. Correlated features that reside in spaces with statistically significant representational similarity (as measured by the main approach discussed in Section \S \ref{sec:methods}) are labeled as \textbf{analogous features} \citep{olah2020zoom}. These similarity measures also measure how much \textit{analogical similarity}, relative to a set of pairings and transformations, each feature has to its paired counterpart. Further discussion of these definitions is provided in Appendix \S \ref{app:univ_vs_true}. 

We do not measure how well models capture \textbf{true features}, which are atomic ground truth features that models may converge towards capturing \citep{ChughtaiToy}. Our hypothesis is that even if SAEs do not capture the same exact features, their features can be matched as \emph{analogous features} that lie in spaces which can be transformed from one to another. 

% we utilize three terms that build on definitions defined in previous works: \textit{correlated features} \citep{bricken2023monosemanticity}, \textit{representational universality} \citep{gurnee2024universalneuronsgpt2language}, and \textit{analogous features} \citep{olah2020zoom}.

% \textbf{Transformer Models.}
% % Embeddings and Positional Encoding, Attention Mechnanism, MLP, Layer Norm, Residual Stream
% Transformer models learn relations across different parts of sequential data by capturing long-range dependencies through the self-attention mechanism \citep{vaswani2017attention}. Each token in an input sequence is first mapped to a fixed-length embedding vector $\mathbf{x}_i \in \mathbb{R}^d$, where $d$ represents the embedding dimension. Since transformers do not inherently capture sequential order, positional encodings $\mathbf{p}_i$ are added to the embeddings.
% % : $\mathbf{z}_i = \mathbf{x}_i + \mathbf{p}_i$.
% The core of the transformer is the self-attention mechanism, which computes attention scores for each token pair using the scaled dot-product attention. 
% % Given a query vector $\mathbf{q}_i$, key vector $\mathbf{k}_j$, and value vector $\mathbf{v}_j$, the attention weights $\alpha_{ij}$ are computed as:
% % \[
% % \alpha_{ij} = \frac{\exp(\mathbf{q}_i^\top \mathbf{k}_j)}{\sum_{k} \exp(\mathbf{q}_i^\top \mathbf{k}_k)}
% % \]
% The output of the attention mechanism is the weighted sum of the values: $\mathbf{y}_i = \sum_{j} \alpha_{ij} \mathbf{v}_j$. This attention process is followed by a position-wise feed-forward network (MLP) and layer normalization to ensure stability.
% % Additionally, a residual connection between input and output overcomes gradient vanishing or exploding issues.

% subsection
\textbf{Sparse Autoencoders.} 
Superposition is a phenomenon in which a model, in response to the issue of having to represent more features than it has parameters, learns feature representations distributed across many parameters \citep{elhage2022superposition}. 
% This leads to issues for interpretability, which aims to disentangle and cleanly identify features in models in order to manipulate them, such as by steering a model away from deception \citep{templeton2024scaling}.
This causes its parameters, or neurons, to be polysemantic, which means that each neuron is involved in representing more than one feature, making it difficult to compare features across different LLMs.
To address this issue, Sparse Autoencoders (SAEs) have been applied to disentangle an LLM's polysemantic neuron activations into monosemantic "feature neurons", which are encouraged to represent an isolated concept.
 % to transform LLM activations into more interpretable spaces spanned by neurons corresponding to individual features.

SAEs are a type of autoencoder that learn sparse representations of input data by imposing a sparsity constraint on the hidden layer  \citep{Makhzani2013kSparseA, cunningham2023sparseautoencodershighlyinterpretable}. 
An SAE takes in LLM layer activations $\mathbf{x} \in \mathbb{R}^n$ and reconstructs $\mathbf{x}$ as output $\mathbf{\hat{x}} = \mathbf{W}'\sigma(\mathbf{W} \mathbf{x} + \mathbf{b})$, where $\mathbf{W} \in \mathbb{R}^{h \times n}$ is the encoder weight matrix, $\mathbf{b}$ is a bias term, $\sigma$ is a nonlinear activation function, and $\mathbf{W}'$ is the decoder matrix, which often uses the transpose of the encoder weights. SAE training aims to both encourage sparsity in the activations $\mathbf{h} = \sigma(\mathbf{W} \mathbf{x} + \mathbf{b})$ and to minimize the reconstruction loss $\left\| \mathbf{x} - \hat{\mathbf{x}} \right\|_2^2$.
% (close to zero) % $\Omega(\mathbf{h})$. 
The sparsity constraint encourages a large number of SAE neuron activations to remain inactive for any given input, while a few neurons, called \emph{feature neurons}, are highly active. 
% Recent work has replaced the regularization term by using the TopK activation function as the nonlinear activation function, which selects only the top K feature neurons with the highest activations \citep{gao2024scalingevaluatingsparseautoencoders}, zeroing out the other activations.
The active feature neurons tend to activate only for specific concepts in the data, promoting monosemanticity.
Therefore, since there is a mapping from LLM neurons to SAE feature neurons that "translates" LLM activations to features, this method is a type of \emph{dictionary learning} \citep{OLSHAUSEN19973311}. Several works make architectural improvements to SAEs \citep{gao2024scalingevaluatingsparseautoencoders, rajamanoharan2024improvingdictionarylearninggated, rajamanoharan2024jumpingaheadimprovingreconstruction}, and analyze its ability to capture LLM features \citep{chanin2024absorptionstudyingfeaturesplitting}. 
% See Appendix \S \ref{app:sae} for more details.

\emph{SAE Feature Weight Spaces. } By analyzing feature weights UMAPs of an SAE trained on a middle residual stream layer of Claude 3 Sonnet, researchers discovered feature spaces organized in neighborhoods of semantic concepts, and identified subspaces corresponding to concepts such as "biology" and "conflict" \citep{templeton2024scaling}. Additionally, these concepts appear to be organized in hierarchical clusters, such as "disease" clusters that contain sub-clusters of specific diseases like flus. In Section \S \ref{sec:subspace_expms}, we measure the extent of similarity of these semantic feature spaces across LLMs.

% When we observe the top 5 or even top 90 highest activating tokens for each neuron in an LLM, there are 

% \textcolor{violet}{} \underline{}
\textbf{Representational Space Similarity.} 
Representational similarity measures typically compare neural network activations by assessing the similarity between activations from a consistent set of inputs  \citep{klabunde2023similarityneuralnetworkmodels}. In this paper, we take a different approach by comparing the representations using the SAE decoder weight matrices \( W' \), whose columns correspond to feature neurons.
We calculate a similarity score \( m(W_X', W_Y') \) for pairs of representations from SAEs $X$ 
We obtain two scores via the following representational similarity measures \footnote{Appendix \ref{app:methodsteps} discusses details on how these measures are applied on decoder weight matrices.}:

\textit{Singular Value Canonical Correlation Analysis (SVCCA)}: 
Given two sets of variables, $\mathbf{X} \in \mathbb{R}^{n \times d_1}$ and $\mathbf{Y} \in \mathbb{R}^{n \times d_2}$, Canonical Correlation Analysis (CCA) seeks to identify pairs of linear transformations $\mathbf{a}$ and $\mathbf{b}$ that maximize the correlation between $\mathbf{X} a$ and $\mathbf{Y} b$ \citep{hotelling1936relations}. 
% called \emph{canonical variables}, $\mathbf{a}_i$ and $\mathbf{b}_i$, 
Singular Value Canonical Correlation Analysis (SVCCA) \citep{Raghu2017SVCCASV} enhances CCA by first applying Singular Value Decomposition (SVD) to both $\mathbf{X}$ and $\mathbf{Y}$ to obtain the left singular matrices $\mathbf{U}_X$ and $\mathbf{U}_Y$ which form orthonormal bases for the column space of their matrices: 

\[
\mathbf{X} = \mathbf{U}_X \mathbf{S}_X \mathbf{V}_X^T, \quad \mathbf{Y} = \mathbf{U}_Y \mathbf{S}_Y \mathbf{V}_Y^T
\]

$\mathbf{S}_X$ and $\mathbf{S}_Y$ are diagonal matrices containing the singular values, and $\mathbf{V}_X^T$ and $\mathbf{V}_Y^T$ contain the right singular vectors.
Dimensionality reduction is applied by truncating low variance directions, which reduces noise, to obtain $\mathbf{U}_{X,k}$ and $\mathbf{U}_{Y,k}$. These represent the principal directions of variance (most informative directions). 

Then, CCA is applied on $\mathbf{U}_{X,k}$ and $\mathbf{U}_{Y,k}$ to find linear transformations $a$ and $b$ that maximize the Pearson correlation between $\mathbf{U}_{X,k} a$ and $\mathbf{U}_{Y,k} b$, such that
% $$
% \rho = \max_{a,b} \frac{a^\top \left(U_{A,k}^\top U_{B,k}\right) b}{\sqrt{a^\top \left(U_{A,k}^\top U_{A,k}\right) a} \sqrt{b^\top \left(U_{B,k}^\top U_{B,k}\right) b}}
% $$
$a$ and $b$ are the canonical directions in each space that are maximally correlated. The SVCCA score is the mean of the top canonical correlations. In other words, it measures how well linear relationships $\mathbf{U}_{X,k} a$ and $\mathbf{U}_{Y,k} b$ align. 
% Therefore, SVCCA measures representation similarity that is invariant to affine transformation. 

% where $\mathbf{U}_X$ and $\mathbf{U}_Y$ are the matrices containing the left singular vectors (informative directions), and $\mathbf{S}_X$ and $\mathbf{S}_Y$ are diagonal matrices containing the singular values. By projecting the original data onto these informative directions, noise is reduced. SVCCA then applies CCA on the transformed datasets, $\mathbf{U}_X$ and $\mathbf{U}_Y$, resulting in correlation scores between the most informative components. These scores are averaged to obtain a similarity score.

% $$
% A = U_A S_A V_A^\top \quad \text{and} \quad B = U_B S_B V_B^\top
% $$

\textit{Representational Similarity Analysis (RSA)}: Representational Similarity Analysis (RSA) \citep{Kriegeskorte2008} has been applied to measure relational similarity of stimuli across brain regions and of activations across neural network layers \citep{klabunde2023similarityneuralnetworkmodels}. First, for each space $\mathbf{X} \in \mathbb{R}^{n \times d_1}$ and $\mathbf{Y} \in \mathbb{R}^{n \times d_2}$, RSA constructs a Representational Dissimilarity Matrix (RDM) $\mathbf{D} \in \mathbb{R}^{n \times n}$, where each element of the matrix represents the dissimilarity (or similarity) between every pair of data points within a space. The RDM essentially summarizes the pairwise distances between all possible data pairs in the feature space. 
For space $\mathbf{X}$, the RDM has entries:
%  of size $n \times n$

$$
  D_{ij}(X) = \|x_i - x_j\|_2,
$$

where $x_i$ and $x_j$ are row vectors (e.g., features). 
% The same calculation is applied to space $Y$ to form $D(X)$ and $D(Y)$. 
A common distance metric used is the Euclidean distance. After an RDM is computed for each space, a correlation measurement like \emph{Spearman's rank correlation coefficient} is applied to the pair of RDMs to obtain a similarity score.
% Then compute the RSA score as:

% $$
% \mathrm{RSA}(X,Y)= \rho_{\text{Spearman}}(D(X), D(Y))
% $$

% \textbf{SVCCA vs RSA. } SVCCA focuses on the comparison of entire vector spaces by aligning the principal components (singular vectors) of two representation spaces and then computing the canonical correlations between them. In other words, it identifies directions in the space that carry the most variance and checks how well these align between two models or layers. On the other hand, RSA is primarily concerned with the structure of relationships, or \emph{relational structure}, between different data points (like stimuli) within a representation space. It allows us to measure how well relations such as king-queen transfer across models.
% Thus, SVCCA focuses on comparing the aligned subspaces of two representation spaces, while RSA is more suitable for analyzing the structural similarity between representations at the level of pairwise relationships.
% For RSA, we are measuring the distances between features. 



==> emnlp_vers/texs/3_methods.tex <==
\section{Methodology}
\label{sec:methods}

% \subsection{Representational Similarity Methods}

% Representational similarity is important for capturing the across-model generalizations of both: 1) Feature Spaces, which are spaces spanned by groups of features, 
% % semantically-related under one common concept
% and 2) Feature Relations.

We compare SAEs trained on layer $A_i$ from LLM $A$ and layer $B_j$ from LLM $B$. This is done for every layer pair.
To compare latent spaces using our selected measures, we have to solve both permutation and rotational alignment issues. For the permutation issue, we have to find a way to pair neuron weights.
This was not an issue in previous representational similarity studies because activations were already paired by input data samples. 
% For example, input $I_k$ is passed through models $A$ and $B$, and then a vector of $N_1$ neuron activations from model $A$ is compared to a paired vector of $N_2$ activations from model $B$. The common input instance creates individual mappings from one space to another, which is required for measures like SVCCA and RSA 
\citep{klabunde2023similarityneuralnetworkmodels}. 
For our case, we do not pair activation vectors by input instances, but pair by feature neuron weights. This means we have to find neuron pairings in SAE $S_A$ to SAE $S_B$ based on individual \emph{local similarity}. However, we do not know which features map to which features; the orderings of these features are permuted in the weight matrices, and some features may not have a corresponding partner. Therefore, we pairwise match them via a correlation metric; a set of pairings is a \emph{mapping}. %, such as by using mean activation correlation. 
For the rotational issue, models learn their own distinct basis for latent space representations, so features may be similar relation-wise across spaces, but not rotation-wise due to differing bases. Thus, we employ rotation-invariant measures. 

\textbf{Assessing Scores with Baseline. } 
% Test 1 follows 
We follow the approach of \citet{Kriegeskorte2008} to randomly pair features to obtain a baseline score. We compare the score of the features paired by correlation (which we refer to as the "paired features") with the average score of $N$ runs of randomly paired features to obtain a p-value score. If the p-value is less than 0.05, the measure suggests that the similarity is statistically meaningful.
The steps to carry out our similarity comparison experiments are given below, and steps 1 to 3 are illustrated in Figure \ref{fig:steps}:
\begin{enumerate}
    \item For the permutation issue: Get activation correlations for SAE decoder weight feature pairs. Pair features from SAE $A$ with its highest activation correlated feature from SAE $B$. 
    \item Rearrange the order of features in each matrix to pair them row by row.
    \item For the rotational issue: Apply rotation-invariant measures to get a \emph{Paired Score}.
    \item Using the same measures, obtain the similarity scores of $N$ \emph{random pairings} to estimate a null distribution. Obtain a p-value of where the paired score falls in the null distribution to determine statistical significance.
    % \item Repeat steps 1 to 3 for LLM activations. If the SAE scores are statistically significant, but the LLM scores are not, then this supports our hypothesis that SAEs can detect feature relation similarities not detectable by LLMs due to superposition.
\end{enumerate}

% For LLMs, given that the neurons are not sparsely activating, we compare the results to SAEs using the top 5, top 30, and top 90 keywords. We use 50 keywords per concept. 

% We use three tests for randomness: 1) permutation shuffling the concept subsets, 2) selecting the same number of random features then taking correlation, and 3) selecting the same number of features from the full space correlation. 

% Test 2 is a variation of Test 1; the change is that instead of randomly shuffling existing pairs, we choose randomly correlated pairs for our subspace. For example, if we find a numerical subspace in each model with 200 1-1 feature pairings, then we generate 100 randomly selected subspace mappings, each with 200 correlated features, by randomly selecting correlated feature pairings, and take the mean score of each subspace mapping. This test shows that the high similarity score does not hold for any subspace of correlated features; in other words, a subspace of features paired by high mean activation similarity do not always yield high SVCCA scores, while a subspace of semantically-related features under a concept does yield a high SVCCA score. % shows not every correlated pairing of subspaces of same size as high score

% \begin{figure*}[!h]
%   \centering
%   \includegraphics[scale=0.43]{diagrams/fig_2_vector.pdf} % 56
%   \caption{Steps to Main Results. We first find correlated pairs to solve neuron permutation, and then apply similarity metrics to solve latent space rotation issues. \textcolor{red}{replace figure - this doesnt look good}}
%   \label{fig:steps}
% \end{figure*}
% %  \hl{will clean this up; may add step 4 }

\textbf{Solving the Permutation Issue:}
% These measures measure individual, local similarity.
Due to variations specific to each LLM and SAE, we do not expect every feature in a SAE to have a corresponding feature that is "close enough" in another SAE. Else, we would forcibly pair features without corresponding partners, yielding low scores due to "bad pairings". Thus, we compare SAE feature subsets.

\emph{Highest Activation Correlation.} We take the activation correlations between every feature, following the approach of \citet{bricken2023monosemanticity}. We pass a dataset of samples through both models. Then, for each feature in SAE $A$, we find its activation correlation with every feature in SAE $B$, using tokens as the common instance pairing. Lastly, for each feature in SAE $A$, we find its highest correlated feature in SAE $B$ (as this allows for many-to-1 mappings, this is termed \textit{1A-to-ManyB}; the other way around is \textit{ManyA-to-1B}). We pair these features together when conducting our experiments. We refer to scores obtained by pairing via highest activation correlation as \emph{Paired Scores}.

% Semantic Similarity
\emph{Filter by Top Tokens.} We notice some pairings with "non-concept features" that have top 5 token activations on end-of-text / padding tokens, spaces, new lines, and punctuation; these non-concept pairings greatly reduce scores possibly due to being "bad pairings", as we describe further in Appendix \ref{app:junk_features}. By filtering out non-concept pairings, we significantly raise the similarity scores. We also only keep pairings that share at least one keyword in their top 5 token activations.
The list of non-concept keywords is given in the Appendix \ref{app:junk_features}.

\emph{Filter Many-to-1 Mappings.}
We find that some mappings are many-to-1, meaning more than one feature maps to the same feature. We found that removing many-to-1 pairings slightly increased the scores, and we discuss possible reasons for this in Appendix \ref{app:1to1}. However, the scores still show high similarity even with the inclusion of many-to-1 pairings. We show scores of 1-to-1 pairings (filtering out many-to-1 pairings) in the main text, and show scores of many-to-1 pairings in Appendix \ref{app:1to1}. 
We choose "many" features from the SAEs of the smaller LLM in a model pair, and find similar results if we choose from SAE of the larger LLM.
% , as seen in Figure \ref{fig:pythia70m_160m_heatmap_both}
% We use features from the SAEs of Pythia-70m and Gemma-1-2B as "many" features which map onto "one" feature in the SAEs of Pythia-160m and Gemma-2-2B.
% Many-to-1 mappings, more so with larger cases like hundreds-to-1, may cause noisy results such as information loss; therefore, we obtain results with less noise by only measuring the subspaces that are mapped 1-1, or are mapped N-to-1, where $N<100$. Hence, we show the 1-1 subspace results in the main text, and put many-to-1 results in the Appendix.

% Removing non-concept features increases several scores in Gemma from around 0.1 to around 0.5. We show in Appendix X the results before removing non-concept features. After removing non-concept features, we retain around half of the features in SAEs. 

% \textbf{Pair by Functional Similarity.} We pair by attribution correlation.

% We pair features 1-1 by the highest activation similarity. Tiebreakers use attribution...

\textbf{Measures for the Rotational Issue}:
Each rotation-invariant measure scores a type of \emph{global, analogous similarity} under a feature mapping. We apply measures for: 1) How well subspaces align using \textbf{SVCCA}, and 2) How similar feature relations like king$\leftrightarrow$queen are using \textbf{RSA}, setting the inner similarity function using Pearson correlation, the outer similarity function using Spearman correlation, and use Euclidean Distance for the RDMs.

\textbf{Semantic Subspace Matching Experiments.}
For these experiments, we first identify semantically similar subspaces, and then compare their similarity. We find a group of related features in each model by searching for features which highly activate on the top 5 samples' tokens that belong to a \emph{concept category}. For example, the "emotions" concept  contains keywords like "rage". 

==> emnlp_vers/texs/4_expms.tex <==

\section{Experiments}

% We compare SAEs of different sizes to observe feature splitting similarities and differences. We also compare SAEs with different properties to check which properties allow for more cross-model feature similarities.

\subsection{Experimental Setup}

% \textbf{Computing Resources.}
We run experiments on an A100 GPU.

\textbf{LLM Models.} We compare LLMs that use the Transformer model architecture \citep{vaswani2017attention}. 
% For comparison robustness due to mean activation correlation pairing by tokens
We compare models that use the same tokenizer because the highest activation correlation pairing relies on comparing two activations using the same tokens.
% We note that certain LLM models may already have similar LLM spaces. Thus, we focus on models which have dissimilar LLM spaces.
% We compare models with a GPT-architecture trained on Tinystories for 1L-21M vs 2L-33M. 
In the main text, we compare the following residual stream layers pairs:
(1) Pythia-70m, which has 6 layers and 512 dimensions, to Pythia-160m, which has 12 layers and 768 hidden dimensions \citep{biderman2023pythiasuiteanalyzinglarge}, and
(2) Gemma-1-2B, which has 18 layers and 2048 dimensions, to Gemma-2-2B, which has 26 layers and 2304 dimensions \citep{gemmateam2024gemmaopenmodelsbased, gemmateam2024gemma2improvingopen}.
% \footnote{Gemma-2 introduces several architectural improvements over Gemma-1 \citep{gemmateam2024gemmaopenmodelsbased, gemmateam2024gemma2improvingopen}.}
% , most notably the addition of Grouped-Query Attention (GQA), which reduces the computational cost of attention while maintaining performance 
% (3) Gemma-2-2B to Gemma-2-9B, which has 42 layers and 3584 dimensions, and (4) Llama 3-8B-Instruct and Llama 3.1-8B, which both have 32 layers and 4096 dimensions.
Appendix \S \ref{app:models} lists all 8 model pairs we compare.

\textbf{SAE Models.} 
% We compare SAEs with the same dictionary size.
% For Tinystories models, we train SAEs on the residual streams for 100k training steps, using ReLU activation function. we used a constant learning rate of $5 \times 10^{-5}$ with no warmup. We calculated the decay steps as 20\% of the total number of training steps to prevent overfitting.
% Hyperparameters: For Models X, 
% observing a loss that plateaus... (discuss SAE losses in Appx)
For Pythia models, we use SAEs with 32768 feature neurons trained on residual stream layers from Eleuther \citep{EleutherAI_sae}.
% ; these SAEs use the TopK activation function, which selects the k largest activations of SAE latents, zeroing the rest \citep{gao2024scalingevaluatingsparseautoencoders}.
For the Gemma models, we use SAEs with 16384 feature neurons trained on residual stream layers \citep{lieberum2024gemmascopeopensparse}.
% , which use the JumpReLu activation function \hl{describe}. 
% These are hosted by
We access pretrained Gemma SAEs
% Gemma-1-2B SAEs for layers 0, 6, 10, 12, and 17, and Gemma-2-2B SAEs for layers 0 to 26, 
through the SAELens library \citep{bloom2024saetrainingcodebase}
% , which only hosted one SAE for Llama 3 at the time of our work.
%icmlAdd

In Appendix \S \ref{app:more_models}, we compare SAEs for Gemma-2-2B vs Gemma-2-9B, base vs fined tuned versions for Gemma-2-9B vs Gemma-2-9B-Instruct and Gemma-1-2B vs Gemma-1-2B-Instruct (at Layer 12), and Llama 3-8B-Instruct vs Llama 3.1-8B. In Appendix \S \ref{app:baseline_to_rand}, we assess a baseline comparison that compares Pythia-70m SAEs with SAEs trained on a randomized Pythia-70m. In Appendix \S \ref{app:withinMod}, we compare SAEs trained within the same model. In Appendix \S \ref{app:cross_model_vary_width}, we compare SAEs across Pythia-70m and Pythia-160m as we vary SAE widths.

% , and compare across base vs fine tuned models, and Llama models \citep{dubey2024llama3, meta2024llama31}, in Appendix \S \ref{app:more_models}. In Appendix \S \ref{app:baseline_to_rand}, we perform a baseline analysis that compares SAEs trained on Pythia-70m to SAEs trained on LLMs with random activations.
% In total, we compare 5 model pairs and find notable similarities across their SAEs. 
% The 8 model pairs we compare are listed in Appendix \ref{app:models}.

\textbf{Datasets.} 
% The Tinystories models are trained on the Tinystories dataset (cite), and 
% The Pythia models are trained on OpenWebText. We also use OpenWebText for our Gemma experiments. The SAEs use the LLM's respective training data to obtain training activations and dataset examples. 
We obtain SAE activations using OpenWebText, a dataset that scraps internet content \citep{Gokaslan2019OpenWebText}. We use 100 samples with a max sequence length of 300 for Pythia for a total of 30k tokens, and we use 150 samples with a max sequence length of 150 for Gemma for a total of 22.5k tokens. Top activating dataset tokens were also obtained using OpenWebText samples. In Appendix \S \ref{app:vary_obtain_actvs}, we vary the dataset and number of tokens used to obtain activations to show that our results do not drastically change when these factors are varied.

%%%%%%%%

% LLM vs 
\subsection{SAE Space Similarity}

In summary, for almost all layer pairs after layer 0, we find the p-value of SAE experiments for SVCCA, which measures rotationally-invariant alignment, to be low; most are between 0.00 to 0.01 using 100 samples.\footnote{Only 100 samples were used as we found the variance to be low for the null distribution, and that the mean was similar for using 100 vs 1k samples.}
While RSA also passes many p-value tests, their values are much lower, suggesting a relatively weaker similarity in terms of pairwise differences.
It is possible that many features are not represented in just one layer; hence, a layer from one model can have similarities to multiple layers in another model.
We also note that the first layer of every model, layer 0, has a very high p-value when compared to every other layer, including when comparing layer 0 from another model. This may be because layer 0 contains few discernible, meaningful, and comparable features.
We find that middle layer pairs have the highest scores. On the contrary, early layers have much lower scores, perhaps due to lacking content, while later layers also have scores lower than middle layers, perhaps due to being too specific/complex.


As shown in Figure \ref{fig:pythia70m_160m_corr_afterFilt_nonconc} for Pythia and Figure \ref{fig:gemma1_2_corr_afterFilt_nonconc} for Gemma-1 vs Gemma-2 in Appendix \ref{app:pythia_full}, we also find that mean of the highest (local) activation correlations does not always correlate with the global similarity measure scores. For instance, a subset of feature pairings with a moderately high mean activation correlation (eg. 0.6) may yield a low SVCCA score (eg. 0.03). 
% We find that for all layers after layer 0, the mean activation correlation pairings differ greatly from the random pairings.
% This often occurs when the features in a subset of pairings are not highly semantically related to one another. 

Because LLMs, even with the same architecture, can learn many different features, we do not expect entire feature spaces to be highly similar; instead, we hypothesize there may be highly similar \emph{subspaces}. In other words, there are many similar features universally found across SAEs, but not every feature learned by different SAEs is the same. Our results support this hypothesis. For all experiments in this section, approximately 10-30\% (and typically 20\%) of feature pairs are kept after filtering both non-concept and Many-1 pairings. 

\textbf{Pythia-70m vs Pythia-160m.}
% \subsubsection{Pythia-70m vs Pythia-160m }
In Figure \ref{fig:pythia70m_160m_heatmap_both_1to1}, we compare Pythia-70m, which has 6 layers, to Pythia-160m, which has 12 layers. When compared to Figures \ref{fig:pythia70m_160m_heatmap_svcca_null} and \ref{fig:pythia70m_160m_heatmap_rsa_null} in Appendix \ref{app:pythia_full}, for all layers pairs (excluding Layers 0), and for both SVCCA and RSA scores, almost all the p-values of the residual stream layer pairs are between 0\% to 1\%, indicating that the feature space similarities are statistically meaningful. In particular, Figure \ref{fig:pythia70m_160m_heatmap_both_1to1} shows that Layers 2 and 3, which are middle layers of Pythia-70m, are more similar by SVCCA and RSA scores to middle layers 4 to 7 of Pythia-160m compared to other layers. 
% sae_pythia_L2
% This pattern is also present with RSA scores in
% in Figure \ref{fig:sae_pythia_rsa_L3} for Layer 3 of Pythia-70m, and in 
% Appendix \ref{app:pythia_full} by Figure \ref{fig:pythia70m_160m_heatmap_rsa_1to1} for Layer 3 of Pythia-70m. 
Figure \ref{fig:pythia70m_160m_heatmap_both} also shows that Layer 5, the last layer of Pythia-70m, is more similar to later layers of Pythia-160m than to other layers.
The number of features after filtering non-concept and many-to-1 features is given in Tables \ref{tab:numfeats_filt_pythia} and \ref{tab:numfeats_unique_pythia} in Appendix \ref{app:pythia_full}.
 % sae_pythia_L5
 
% In contrast, for LLMs, the tests indicate no statistical significance. This implies that SAEs can detect feature relation similarities not detectable by LLMs due to superposition. 
% % While LLMs still contain some highly similar neuron pairs, 

% \begin{figure*}[!h]
%   \centering
%   \includegraphics[scale=0.4]{diagrams/L2vL3pythia.png} % sae_pythia_L2
%   \caption{SVCCA 1-1 scores of SAEs of layer 2 in Pythia-70m vs all layers in Pythia-160m. The blue bars indicate SVCCA scores of Paired Scores, and the orange bars indicate mean scores of random pairings. We note L2 (a middle layer) of Pythia-70m is more similar to the middle layers of Pythia-160m.}
%   \label{fig:sae_pythia_L2}
% \end{figure*}

\begin{figure*}[!h]
  \centering
  % \includegraphics[scale=0.28]{diagrams/pythia70m_160m_heatmap_both.pdf}
  \includegraphics[scale=0.275]{diagrams/pythia70m_160m_heatmap_both_1to1.pdf}
  % LLMs vs 
  % \caption{(a) SVCCA and (b) RSA paired scores of SAEs for layers in Pythia-70m vs layers in Pythia-160m. We find that middle layers have the most similarity with one another (as shown by the high-similarity block spanned by Layers 1 to 3 in Pythia-70m and Layers 4 to 7 in Pythia-160m). We exclude layers 0, as we observe they always have non-statistically significant similarity. We note there appears to be an "anomaly" at L2 vs L3 with a low SVCCA score; we find that taking 1-1 features greatly increases this score from 0.03 to 0.35, as shown and explained in Figure \ref{fig:pythia70m_160m_heatmap_both_1to1} in  Appendix \ref{app:1to1}. }
  \caption{(a) SVCCA and (b) RSA 1-1 paired scores of SAEs for layers in Pythia-70m vs layers in Pythia-160m. We find that middle layers have the most similarity with one another (as shown by the high-similarity block spanned by layers 1 to 3 in Pythia-70m and Layers 4 to 7 in Pythia-160m). We exclude layers 0, as we observe they always have non-statistically significant similarity. The 1-1 scores are slightly higher for most of the Many-to-1 scores shown in Figure \ref{fig:pythia70m_160m_heatmap_both}, and the SVCCA score at L2 vs L3 for 70m vs 160m is much higher. }
  % \label{fig:pythia70m_160m_heatmap_both}
  \label{fig:pythia70m_160m_heatmap_both_1to1}
\end{figure*}
% As these scores are much higher than randomly paired scores in Figures \ref{fig:pythia70m_160m_heatmap_svcca_null} and \ref{fig:pythia70m_160m_heatmap_rsa_null} in Appendix \ref{app:1to1}, and the p-values for most layer pairs are below 0.05, we find statistically meaningful feature space similarities. 

%%%%%%%
\textbf{Gemma-1-2B vs Gemma-2-2B. } 
% \subsubsection{Gemma-1-2B vs Gemma-2-2B}
% , making it faster and more efficient during inference. 
% It also implements both pre-norm and post-norm strategies for better training stability, unlike Gemma 1, which uses a more traditional transformer normalization. Gemma 2 further incorporates knowledge distillation, allowing smaller models to learn from larger teacher models, significantly improving performance (to cite).
% Table \ref{tab:gemma_svcca}
% Gemma1-2B Layer 12 vs Gemma2-2B Layer 15 has a SVCCA score of 0.54, compared to 0.004 for the average of random runs. 
% As shown in Figure \ref{fig:sae_gemma_L12},
As shown by the paired SVCCA and RSA results for these models in Figure \ref{fig:gemma1_gemma2_heatmap_both_1to1}, we find that using SAEs, we can detect highly similar features in layers across Gemma-1-2B and Gemma-2-2B. Compared to mean random pairing scores and p-values in Figures \ref{fig:gemma1_2_heatmap_svcca_null} and \ref{fig:gemma1_2_heatmap_rsa_null} in Appendix \ref{app:pythia_full}, for all layers pairs (excluding Layers 0), and for both SVCCA and RSA scores, almost all the p-values of the residual stream layer pairs are between 0\% to 1\%, indicating that the feature space similarities are statistically meaningful.
The number of features after filtering non-concept features and many-to-1 features are given in Tables \ref{tab:numfeats_filt_gemma} and \ref{tab:numfeats_unique_gemma} in Appendix \ref{app:pythia_full}.

\begin{figure*}[ht]
  \centering
  % \includegraphics[scale=0.275]{diagrams/gemma1_gemma2_heatmap_both.pdf}
  \includegraphics[scale=0.275]{diagrams/gemma1_gemma2_heatmap_both_1_1.pdf}
  % LLMs vs 
  \caption{(a) SVCCA and (b) RSA 1-1 paired scores of SAEs for layers in Gemma-1-2B vs layers in Gemma-2-2B. Middle layers have the best performance. The later layer 17 in Gemma-1 is more similar to later layers in Gemma-2. Early layers like Layer 2 in Gemma-2 have very low similarity. We exclude layers 0, as we observe they always have non-statistically significant similarity. The 1-1 scores are slightly higher for most of the Many-to-1 scores shown in Figure \ref{fig:gemma1_gemma2_heatmap_both}. }
  % \label{fig:gemma1_gemma2_heatmap_both}
  \label{fig:gemma1_gemma2_heatmap_both_1to1}
\end{figure*}
% Compared to Figures \ref{fig:gemma1_2_heatmap_svcca_null} and \ref{fig:gemma1_2_heatmap_rsa_null} in  Appendix \ref{app:1to1}, some of the scores are slightly higher.

% \textbf{Gemma-2-2B vs Gemma-2-9B.}
% % \label{app:gemma9b}
% % We compare Gemma-2-2B vs Gemma-2-9B at several layers of each model, which each have 25 and 41 layers, respectively. Each SAE has a width of 16384 features and uses JumpReLU \citep{rajamanoharan2024jumpingaheadimprovingreconstruction}, and is hosted on SAELens. 
% We obtain activations from OpenWebText using 150 samples with a max sequence length of 150, for a total of 22.5k tokens. Figure \ref{fig:gemma2b_gemma9b_heatmap_both_1to1} shows SVCCA and RSA scores after filtering keywords and for 1-1. In particular, the L11 vs L21 comparison achieves an SVCCA score of 0.70 (while mean random pairing has a score of 0.009) and an RSA score of 0.195 (while mean random pairing for has a score of $4.38 \times 10^{-4}$). For these experiments, we use 10 runs for mean random pairings at only one layer pair due to the longer run times for larger model pairs.
% %  the L13 vs L22 comparison achieves an SVCCA score of 0.65 (while mean random pairing has a score of 0.2) and an RSA score of 0.15 (while mean random pairing has a score of $-1.49 \times 10^{-5}$).

% \begin{figure*}[ht]
%   \centering
%   \includegraphics[scale=0.275]{diagrams/gemma2b_gemma9b_heatmap_both_1to1.pdf}
%   % LLMs vs 
%   \caption{(a) SVCCA and (b) RSA 1-1 paired scores of SAEs for layers in Gemma-2-2B vs layers in Gemma-2-9B. Middle layers have the best performance. We exclude layers 0, as we observe they always have non-statistically significant similarity. }
%   \label{fig:gemma2b_gemma9b_heatmap_both_1to1}
% \end{figure*}

% \textbf{Llama 3-8B-Instruct vs Llama 3.1-8B . }
% We compare Llama 3-8B-Instruct and Llama 3.1-8B at each model's Layer 25 residual stream, a later layer in both models. We obtain activations using 100 samples with a max sequence length of 100, for 10000 total tokens. After filtering to keep 7\% of Llama 3.1-8B feature pairs, this comparison achieves an SVCCA score of 0.3, comparable to the score of later layers in both Gemma and Pythia, and a mean activation correlation score of 66\%.

% \subsubsection{Similarity of Semantically Matched SAE Feature Spaces}
\subsection{Similarity of Semantic SAE Subspaces}
\label{sec:subspace_expms}

% First, we find features from each model that, in their top 5 activating tokens, activate on the keywords belonging to the concept group for at least 3 out of 5 samples. Then, we pair these features using max activation correlation, filtering out many-to-1 matches and those with low correlation. We manually check if the paired interpretations are truly activating on similar keywords belonging to the concept group. Finally, we take the metric scores and compare these to random shuffling of the pairs.

% We find that for all layers and for all concept categories, Test 2 described in \S \ref{sec:methods} is passed. Thus, we only report specific results for Test 1 in Tables \ref{tab:subspace_expms_1} and \ref{tab:subspace_expms_gemma_svcca}.
% We also test on several groups of unrelated keywords, manually inspecting to check that each word belongs to its own category. These result in high p-values, suggesting that subspaces are found universally when the features in a subspace are more semantically related to one another \hl{put in appendix}. 
Overall, in both Pythia and Gemma models and for many concept categories, we find that semantic subspaces are more similar to one another than non-semantic subspaces. More discussion on these results is given in Appendix \ref{app:categ}.

Rather than just finding that middle layers are more similar, we find that they are the best at representing concepts. This is consistent with work by \citep{rimsky2024steering}, which find the best steering vectors in middle layers for steering behaviors such as sycophancy.
Other papers find that middle layers tend to provide better directions for removing refusal behavior \citep{arditi2024refusal} and work well for representing goals and finding steering vectors in policy networks \citep{mini_understanding_2023}.

\textbf{Pythia-70m vs Pythia-160m. } 
% \subsubsection{Pythia-70m vs Pythia-160m} 
We compare every layer of Pythia-70m to every layer of Pythia-160m for several concept categories. While many layer pairs have similar semantic subspaces, middle layers appear to have the semantic subspaces with the highest similarity.
Table \ref{tab:subspace_expms_1} demonstrates one example of this by comparing the SVCCA score for layer 3 to layer 5 of Pythia-160m, which shows high similarity for semantic subspaces across models, as the concept categories all have p-values below 0.05.
We show the scores for other layer pairs and categories in Figures \ref{fig:svcca_heatmaps_concepts_pythia} and \ref{fig:rsa_heatmaps_concepts_pythia} in Appendix \ref{app:pythia_full}, which include RSA scores in Table \ref{tab:subspace_expms_rsa_l3_l5}. 
% and the top 5 snippets each feature in the subset highly activates on 
% , passing both tests in comparison to null distributions.

% We observe that middle layers tend to have the most detectable features, while later layers do not. The p-values of the middle layers like L5 in Pythia-160m all indicate statistical significance for all concept groups, but for the late layers like L10 in Pythia-160m, only concept groups of 'science' and 'nature' have plentiful features (a few hundred) with across-model similarity p-values indicating statistical significance. This may be because later layers contain more “complex and composite” features, while features like numerical and people-related are more like "abstract building blocks". However, this is just our hypothesis which we did not test in this study.

% In comparison, for most categories and layer pairs, attempting to get top dataset examples from LLM neurons to extract semantic subspaces results in high p-values. This occurs whether we allow keywords to be in the top 5, top 30, or top 90 dataset example tokens. of note is that the numeric category appears to be more monosemantic in the LLMs. This is because some neurons in some LLMs are already monosemantic; however, the vast majority are not.

% %  (may be RSA side-by-side with this)
% \begin{table*}
%     \centering
%     \caption{ SVCCA scores and random mean results for 1-1 semantic subspaces of L3 of Pythia-70m vs L5 of Pythia-160m. P-values are taken for 1000 samples in the null distribution.}
%     \label{tab:subspace_expms_1}
%     \vspace{0.5em}
%     \begin{tabular}{c|cccc}
%         \toprule
%         Concept Subspace & Number of Features &  Paired Mean & Random Shuffling Mean & p-value \\
%         \midrule
%         Time & 228 & 0.59 & 0.05 & 0.00 \\
%         Calendar & 126 & 0.65 & 0.07 & 0.00 \\
%         Nature & 46 & 0.50 & 0.12 & 0.00 \\ % 0.001
%         % MonthNames & 32 & 0.72 & 0.14 & 0.00 \\
%         Countries & 32 & 0.72 & 0.14 & 0.00 \\
%         People/Roles & 31 & 0.50 & 0.15 & 0.00 \\ % 0.007
%         Emotions & 24 & 0.83 & 0.15 & 0.00 \\
%         \bottomrule
%     \end{tabular}    
% \end{table*}

% % After filtering out those below 0.4: Numerical: paired is 0.42, random is 0.13. P-value for 10k random runs is 0.01.

\textbf{Gemma-1-2B vs Gemma-2-2B. } 
% \subsubsection{Gemma1 vs Gemma2}
In Table \ref{tab:subspace_expms_gemma_svcca}, we compare  L12 of Gemma-1-2B vs L14 of Gemma-2-2B. As shown in Figure \ref{fig:gemma1_gemma2_heatmap_both}, this layer pair has a very high similarity for most concept spaces; as such, they likely have high similar semantically-meaningful feature subspaces. 
Notably, not all concept groups are highly similar; for instance, unlike in Pythia, the Country concept group has a p-value above 0.05. 
% While all measured concept groups are highly similar, there is one concept group which does not- month names. Unlike in Pythia, the month names subspace is not highly similar. (continue analysis here)
We show the scores for other layer pairs and categories in Figures \ref{fig:svcca_heatmaps_concepts_gemma} and \ref{fig:rsa_heatmaps_concepts_gemma} in Appendix \ref{app:pythia_full}.

% \begin{table*}[!h]
%     \centering
%     \caption{SVCCA scores and random mean results for 1-1 semantic subspaces of L12 of Gemma-1-2B vs L14 of Gemma-2-2B. P-values are taken for 1000 samples in the null distribution. }
%     \label{tab:subspace_expms_gemma_svcca}
%     \vspace{0.5em}
%     \begin{tabular}{c|cccc}
%         \toprule
%         Concept Subspace & Number of Features & Paired SVCCA & Random Shuffling Mean & p-value \\
%         \midrule
%         Time & 228 & 0.46 & 0.06 & 0.00 \\
%         Calendar & 105 & 0.54 & 0.07 & 0.00 \\
%         Nature & 51 & 0.30 & 0.11 & 0.01 \\
%         % MonthNames & 44 & 0.01 & 0.12 & 0.99 \\
%         Countries & 21 & 0.39 & 0.17 & 0.07 \\
%         People/Roles & 36 & 0.66 & 0.15 & 0.00 \\
%         Emotions & 35 & 0.60 & 0.12 & 0.00 \\
%         \bottomrule
%     \end{tabular}    
% \end{table*}


==> emnlp_vers/texs/5_relatedwork.tex <==
\section{Related Work}

% \textbf{Superposition and Sparse Autoencoders. } Superposition is a phenomenon in which a model, in response to the issue of having to represent more features than it has parameters, learns feature representations distributed across many parameters \citep{elhage2022superposition}. This causes its parameters, or neurons, to be polysemantic, which means that each neuron is involved in representing more than one feature. This leads to issues for interpretability, which aims to disentangle and cleanly identify features in models in order to manipulate them, such as by steering a model away from deception \citep{templeton2024scaling}. To address the issue of polysemanticity, Sparse Autoencoders (SAEs) have been applied to disentangle an LLM's polysemantic neuron activations into monosemantic "feature neurons", which are encouraged to represent an isolated concept \citep{Makhzani2013kSparseA, cunningham2023sparseautoencodershighlyinterpretable, gao2024scalingevaluatingsparseautoencoders, rajamanoharan2024improvingdictionarylearninggated, rajamanoharan2024jumpingaheadimprovingreconstruction}. Features interactions in terms of circuits have also been studied \citep{marks2024sparse}.

% , finding that SAE feature correlations are stronger than LLM neuron correlations; 
% To the best of our knowledge, only 
\textbf{Feature Universality. } Previous works studied universality in terms of components such as features and circuits \citep{olah_batson_2023_feature, ChughtaiToy}. \citet{bricken2023monosemanticity} measure individual SAE feature similarity for two 1-layer toy models; however, this study did not analyze the global properties of feature spaces. \citet{gurnee2024universalneuronsgpt2language} find evidence of universal neurons across language models by applying pairwise correlation metrics.
% , and taxonimized families of neurons based on patterns of downstream, functional effects.
\citet{oneill2024disentanglingdenseembeddingssparse} discover "feature families" representing related hierarchical concepts in SAEs across semantically different datasets.
\cite{huh2024platonic} showed that as vision and language models are trained with more parameters and with better methods, their representational spaces converge towards more similar representations. 
Crosscoders  \citep{lindsey2024sparse, mishrasharma2025insights} and Universal SAEs \citep{thasarathan2025universalsparseautoencodersinterpretable} are SAE variations that capture individual features shared across models.
% In this paper, we do not claim nor attempt to study if models converge towards finding the same features.
% as explained in Appendix \S \ref{app:univ_vs_true},
% SAEs may also converge to similar representations.
% One hypothesis is that LLMs trained on SAEs may also converge to similar representations as the LLMs or SAEs are trained with more parameters and with better methods.

% varying levels of abstraction
% The authors state "Visualizing the resulting principal components confirms that the feature families we find do not represent manifolds or irreducible multi-dimensional structures. We can instead think of feature families as linear subspaces". The feature families they find (across 2 dataset embeddings) appear to be linear subspaces; however, this does not mean all interesting structures would be linear subspaces. Regardless, there remains much to be explored with linear subspace structures, which our paper also looks for, even if manifold structures are not found.

\textbf{Representational Space Similarity. } Previous work has studied neuron activation spaces by utilizing metrics to compare the geometric similarities of representational spaces \citep{Raghu2017SVCCASV, wang2018understanding, kornblith2019similarityneuralnetworkrepresentations, klabunde2024resicomprehensivebenchmarkrepresentational, klabunde2023similarityneuralnetworkmodels, Kriegeskorte2008, SucholutskyAligned}, finding that even models with different architectures may share similar representation spaces, hinting at feature universality. 
However, these techniques have yet to be applied to the feature spaces of SAEs trained on LLMs. Moreover, these techniques compare the similarity of paired input activations. Our work differs as it compares the similarity of paired \emph{feature weights}. Essentially, previous works do not show that one can match LLMs by features learned by both LLMs.
For vision models, \cite{kondapaneni2025representational} discover shared and unique visual concepts between different models.

% Additionally, these studies applied these techniques to neurons that are likely highly polysemantic, and thus, their feature spaces may not as cleanly separated into clusters as SAE feature space, in which features are more likely to be monosemantic and sparse. Thus, as they study polysemantic neurons, these works may not have been able to cleanly find evidence for analogous feature subspaces. 
% Understanding SAE feature space similarity can shed even greater light on feature manifolds and feature relation universality.

% \textbf{Feature Manifolds. } In real world data, features may lie on a manifold, where nearby features respond to similar data. \citep{olah_batson_2023_feature, bricken2023monosemanticity}. Previous work has discovered the existence of features corresponding to months and days of the week arranged in a circular structure in SAE feature spaces across models \citep{engels2024languagemodelfeatureslinear}. Studying how feature arrangements generalize across models may shed light on how features lie on a manifold.

% This is early evidence that features may be arranged in topological patterns- such as circles, trees, or tori- that can be identified across models. These topological patterns may characterize feature subspaces that correspond to semantically similar concepts. Indeed, other works have examined the activation spaces of neurons and discovered topological structures such as loops and branches formed by semantically similar concepts like "animal" or "face" that suggest the existence of feature manifolds \citep{carter2019activation, rathore2021topoact, rathore2023topobert}. 

% in the causal inner product space, which unifies the last-token-last-layer embedding space and the unembedding space, of a LLM (Gemma-2B) 
% Lastly, geometric structures such as simplices have been discovered in an LLM \citep{park2024geometry}. However, finding these structures has yet to be studied for the intermediate spaces of LLMs.
% ; we also investigate the existence of these higher-order structures in our paper.

% \textbf{Manifold Approximation Methods. } Methods such as Mapper, a technique from the field of Topological Data Analysis, have been applied to approximate feature manifolds in the neuron representation spaces of image and language models \citep{rathore2021topoact, rathore2023topobert}. These methods have yet to be applied to the feature spaces of SAEs.

% Multi-Scale Intrinsic Distance \citep{TsitsulinMMKBOM20} and the Geometry Score \citep{Khrulkov2018}

% \textbf{Functional Similarity. } (Discuss mech interp and circuits + steering vectors found across models here)

% Functionally equivalent features... \citep{chen2023goingneuralnetworkfeature}... however, these methods have not been applied to SAE features yet.

% garde2023deepdecipheraccessinginvestigatingneuron
\textbf{Mechanistic Interpretability. } 
Previous work has made notable progress in neuron interpretation \citep{foote2023neurongraphinterpretinglanguage} and interpreting the interactions between components \citep{neo2024interpretingcontextlookupstransformers}.
% (to finish adding to soon)
Other work in mechanistic interpretability focus on circuits analysis \citep{elhage2021mathematical}, as well using steering vectors to control model behaviors \citep{zou2023representation, turner2023activation}.
% ; see representation engineering \citet{zou2023representation} and activating engineering \citep{turner2023activation}, along with \citet{bereska2024mechanisticinterpretabilityaisafety} for a more thorough overview. Notably, steering methods are not limited to LLMs and instead can work on other networks such as policy networks \citet{mini_understanding_2023}. 
These approaches have been combined with SAEs to steer models in the more interpretable SAE feature space \citep{chalnev_improving_2024}. Steering vectors have been found across models, such as vectors that steered a model to refuse harmful instructions across 13 different models \citep{arditi2024refusal}. 
% , including Gemma and Llama-2. 
% This suggests that steering vectors may be found universally across LLMs.
% bereska2024mechanisticinterpretabilityaisafety
% nanda2024decompsae

% to be incl. - sleeper agents paper, ngo's alignment from deep learning perspective, hubinger model organism approach, mrinank's sycophancy paper, 
% work in model organisms potentially? not fitting with the flow, leave out for now

% recent alignment faking paper may be good addition - check with michael before adding here
\textbf{AI Safety. }
Advanced AI may not be aligned with the values of their designers \citep{ngo_alignment_2022}, due to phenomena such as goal misgeneralization \citep{shah_goal_2022}, deceptive alignment \citep{greenblatt_alignment_2024}, and reward tampering \citep{denison_sycophancy_2024}. 
SAEs can find steerable safety-related features across models, such as refusal features \citep{obrien2024steeringlanguagemodelrefusal}. Finding reliable universal capabilities and control methods, like in SAEs, helps provide solutions to safety issues.
% especially in combination with control methods such as steering,
% langosco_goal_2022
% hubinger_risks_2021 hubinger_sleeper_2024
% sycophancy \citep{sharma_towards_2023},

% focus on deceptive capabilites and how SAEs can help tease out across different models, below
% can argue that universal feat. repr.s include shared deceptive capabilities in a general sense, but better to have a key citation or two to shore up that point. add tomorrow







==> emnlp_vers/texs/6_conclusion.tex <==
\section{Conclusion}

%  Our primary goal is to measure the extent of similarity between SAE features across different LLMs. 
In this study, we take the first steps in investigating the unexplored topic of feature space universality in LLMs via sparse autoencoders (SAEs) trained on different models. To achieve these insights, we developed a novel methodology to pair features with high activation correlations, and then assess the global similarity of the resulting subspaces using SVCCA and RSA. 
Our findings reveal a high degree of SVCCA similarity in SAE feature subspaces across various models, particularly between their middle layers.
% Our findings reveal a high degree of similarity in SAE feature spaces across various models when evaluated through SVCCA, indicating robust rotation-invariant space alignment. When analyzing these spaces through RSA, which focuses on pairwise differences, we observed a relatively weaker similarity. This discrepancy highlights the complexity and variability in feature space representation across different models and semantic contexts.
Furthermore, our research reveals that subspaces of features associated with specific semantic concepts, such as calendar or people tokens, demonstrate remarkably high similarity across different models. This suggests that certain semantic feature subspaces may be universally encoded across varied LLM architectures. However, our results also show that there are parts of SAE feature spaces which do not match, and may suggest that either certain features are not captured universally, or that SAEs have limitations in capturing universal features. We believe that future work can benefit from these discoveries to find better ways on improving methods to capture feature universality.
% Our work enhances understanding of how LLMs represent information at a fundamental level, opening up new avenues for further research into model interpretability and the transferability of learned features.
% Our work opens up several exciting avenues for future research. Exploring whether universal features can be leveraged to improve transfer learning or model compression techniques may lead to more efficient training paradigms \citep{Yosinski2014, Hinton2015DistillingTK}. 
% do not consistently learn the same exact features captured by LLMs
Lastly, while we discover evidence that LLMs learn "weakly universal" features, and that SAEs can capture both these features and these relations, we also find that there is a notable fraction of features idiosyncractic to different SAEs, a finding that is supported by previous work \citep{leask2025sparse, paulo2025sparseautoencoderstraineddata}. Thus, our research guides future work to improve upon methods that can better capture universal feature representations, and contributes to ongoing research that aims to improve SAEs \citep{engels2024decomposingdarkmattersparse}. Our approach may be generalized to compare feature spaces beyond those of SAEs.
% \citep{thasarathan2025universalsparseautoencodersinterpretable}

Examining the implications of feature universality for AI safety and control, particularly in identifying and mitigating potentially harmful representations, can contribute to the development of safer AI systems \citep{barez2023iii}. 
% By shedding light on the internal representations of LLMs, our research contributes to the broader goal of developing more interpretable, efficient, and reliable AI systems \citep{barez2023iii}. 
Overall, understanding the commonalities and differences in model representations is a crucial step towards a more comprehensive theory of how models generate human language.

% \begin{enumerate}
%     \item Main Research Problem: SAE feature universality is an underexplored topic, as no work has been done so far in comparing the features spaces of SAEs trained on LLMs with more than one layer and for more than one pair of LLMs, nor has work been done in comparing the spatial and relational properties of SAE feature spaces.
%     \item Main Goal: We measure the extent of similarity between SAE features across LLMs. 
%     \item Main Finding: We find that SAE feature spaces are highly similar across models in terms of SVCCA (rotation-invariant space alignment). We find weaker similarity between SAE feature spaces in terms of RSA (pairwise differences).
%     \item Secondary Finding: We find that subspaces of features belonging to a semantic concept (eg. numeric, people, etc.) are highly similar across models.
%     \item Method Summary: We devise a statistical test to find similar subspaces across models. This involves pairing highly similar individual features by mean activation correlation, and then measuring the global similarity of the subspaces spanned by those features using SVCCA and RSA.
% \end{enumerate}

\section*{Limitations}
% available pre-trained 
We perform analysis only on a sample of SAEs for similar LLMs that use the same tokenizer, and focus on SAEs with the same or similar number of features.
As we pair features by activation correlation, we do not perform analysis on models that use different tokenizers. Although, for some examples, we obtain good results when pairing featuers only by semantic similarity, these results were not consistent when applied to other examples, perhaps due to the lower pairing quality, as the representational similarity measures depend on the pairing choice. Future work can analyze models whose representations do not depend as much on the tokenizer choice \citep{lcmteam2024largeconceptmodelslanguage}.

% However, there are a limited number of pre-trained SAEs on large models. 
Our study is also limited by the inherent challenges in interpreting and comparing high-dimensional feature spaces. The methods we used to measure similarity, while robust, may not capture all nuances of feature interactions and representations within the SAEs. Additionally, our analysis is constrained by the computational resources available, which limited our activations dataset sizes, along with the scale and depth of our comparisons. The generalizability of our findings to SAEs trained on more diverse datasets or specialized domain-specific LLMs remains an open question. Lastly, our analysis does not account for potential temporal dynamics in feature representation that may occur at different training stages of LLMs and SAEs. 
% Lastly, functional similarity experiments were not examined.

% \section*{Impact Statement}
% Our study investigates feature universality in large language models (LLMs) using sparse autoencoders (SAEs) to identify common feature spaces across models. This research contributes to safety research by providing insights into how different LLMs encode safety-related concepts, which has several ethical and societal implications.
% By identifying universal feature spaces, our approach may aid in the detection of harmful or deceptive model behaviors across different architectures. Understanding how models encode knowledge could lead to improved transparency and control mechanisms, reducing risks associated with goal misgeneralization and deceptive alignment in AI systems. Additionally, identifying shared feature structures can inform bias mitigation strategies, as universal features could either amplify or help detect biases present across multiple models.

% Universal features enable transfer learning and model compression, boosting AI efficiency and accessibility. However, they also raise ethical concerns—such as model replication, knowledge extraction, and adversarial attacks—which require further research to ensure responsible use. These findings deepen our understanding of LLM representations and bear implications for AI safety, fairness, and alignment.

% \section*{Future Work}
% Future work can compare LLMs to SAEs. Early work we have conducted has applied similar analysis on the LLMs that the SAEs in this paper were trained on, and found that they have some similarity, but much lower than that of the SAEs, with no patterns showing that the middle layers were the most similar. 
% Additionally, the LLMs did not have corresponding weights for the "residual stream", which is an addition of activations from the MLP and attention head layers, so we compared the MLPs of LLMs. Unlike the SAE dimensions, the MLP dimensions of the LLMs had different dimensions. Future work could study the comparison of LLM similarity by feature weights to SAEs. Additional experiments could include ground-truth feature experiments which examine LLMs that partially share ground-truth features to see if SAEs are modeling the same features \citep{sharkey2022interim}, and functional similarity experiments \citep{bricken2023monosemanticity}.

% \section*{Author Contributions}
% \label{sec:contributions}
% Michael conceived the study and designed the experiments with help from Fazl. Michael performed the experiments with help from Austin and led the writing of the manuscript. Philp, Ashkan and David provided advice throughout the project. 
% Fazl advised this work and helped significantly with the write-up of the paper.

% \section*{Acknowledgments}
% We thank the Torr Vision Group at the University of Oxford for providing compute and hosting Michael Lan during the internship.
% We thank Clement Neo, Luke Marks, Minseon Kim, Lovis Heindrich, Tingchen Fu, Constantin Venhoff, Hazel Kim, Will Lin, Alasdair Paren, Christian Schroeder de Witt, Kiho Park, and Max Klabunde for providing helpful feedback. Clement Neo helped with the design of Figure 1.

% \section*{Reproducibility}
% We include the code and instructions for reproducing our main results in the Supplementary Materials.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

